Exploring SU(3)-Higgs theories

The requirement of manifest gauge invariance leads to a conflict between perturbative and non-perturbative predictions for the low-energy spectra of grand-unified theories. These conflicts already emerge in simplified prototype models of SU(3) gauge theories with Higgs fields in different representations. We expand earlier lattice investigations on this subject and provide further support for the predicted deviations. These can be understood in terms of the Froehlich-Morchio-Strocchi mechanism.

==> extra/app-constructing-ops.tex <==
\section{Constructing a basis of operators}
\EDil{not sure if this is actually worth including as it seems like too much information and doesn't add anything in terms of physics. Just wrote this because it was the easiest thing to describe, but feel free to remove if unnecessary.}
In order to construct a suitable basis of operators to probe all accessible channels, we follow an approach closely based on that of \cite{dudek2010}. In the following we denote channels by their quantum numbers $J^{PC}_G$ with $J\in\{0,1,2\}$ the total continuum spin, $P\in\{+1,-1\}$ the parity, $C\in\{+1,-1\}$ the charge parity, and $G$ the charge corresponding to the custodial symmetry -- in this case, $\U[1]$.

We assume, for now, that any state of interest on the lattice can be described as a discretised version of an operator that is local in the continuum limit.\footnote{some comment about this} Define the operators $\alpha$ and $\beta$ respectively, as a `string' of $N$ covariant derivatives dressed by a pair of scalar fields, and a triple product of scalar fields acted upon by covariant derivatives:
\footnote{Here roman indices denote (colour) components of the 3-component vectors}
\begin{gather}
    \alpha_{\mu_1,\dots,\mu_N}(x) 
    = \phi^\dag(x) (D_{\mu_N}D_{\mu_{N-1}}\dots D_{\mu_1}\phi)(x)\;,
    \\
    % \beta_{\substack{\mu_1,\dots,\mu_{N_\mu}\\\nu_1,\dots,\nu_{N_\nu}\\\rho_1\dots,\rho_{N_\rho}}}(x) 
    % = \epsilon_{abc}
    % (D_{\rho_{N_\rho}}\dots D_{\rho_1}\phi)_a (x)
    % (D_{\nu_{N_\nu}}\dots D_{\nu_1}\phi)_b (x)
    % (D_{\mu_{N_\mu}}\dots D_{\mu_1}\phi)_c(x)\;.
    \beta_{\mu_1,\dots,\mu_{N};\{r,s\}}(x) 
    = \epsilon_{abc}
    (D_{\mu_N}\dots D_{\mu_{s+1}}\phi)_a (x)
    (D_{\mu_{s}}\dots D_{\mu_{r+1}}\phi)_b (x)
    (D_{\mu_{r}}\dots D_{\mu_1}\phi)_c(x)\;.
\end{gather}

% While in principle there are of course infinitely many possible operators, there is reason to suspect that operators with minimal field content are the most relevant for now, so we restrict attention to linear combinations of either $\alpha$ or $\beta$ operators, along with scattering operators constructed from their products. 
To construct an operator in a relevant channel on the lattice, we then first look for a linear combination of either $\alpha$ or $\beta$ operators corresponding to a given value of continuum spin $J$. On the lattice, this can be done most intuitively by working with `ladder operators' on each spatial timeslice%
\footnote{
Here $\hat{D}_i$ with $i\in\{1,2,3\}$ denotes the standard spatial components of the lattice-discretised form of $D_\mu$, i.e:\\\hspace*{2em}
\mbox{$\displaystyle
    \hat{D}_\mu \hat{\phi}(x)=\frac{1}{2}\bq*{U_{\mu}(x)\phi(x+a\emu) - U^\dag_{\mu}(x-a\emu)\phi(x-a\emu)} \,.
$}
}:
\begin{equation}
    \wt{D}_{\pm 1}=\mp\frac{i}{\sqrt{2}}(\hat{D}_1\pm i \hat{D}_2),\qquad
    \wt{D}_0 = i \hat{D}_3\,,
\end{equation}
and looking for linear combinations of either
\begin{gather}
    \wt{\alpha}_{m_1,\dots,m_N}(x)=\hat\phi^\dag(x)(\wt{D}_{m_N}\dots \wt{D}_{m_1}\phi)(x)\,,
    \quad\text{or}\quad
    \\
    \wt{\beta}_{m_1,\dots,m_{N}; \{r,s\}}(x) = \epsilon_{abc} 
    (\wt{D}_{m_N}\dots\wt{D}_{m_{s+1}}\hat\phi)_a(x)
    (\wt{D}_{m_s}\dots\wt{D}_{m_{r+1}}\hat\phi)_b(x)
    (\wt{D}_{m_r}\dots\wt{D}_{m_{1}}\hat\phi)_c(x)\,.
\end{gather}
% with a fixed number of indices, 
% depending on whether we are interested in states that are neutral or charged under the custodial $\U[1]$ symmetry.

Such a linear combination, $\cO^{J,M}_{[j'_2,\dots,j'_{(N-1)}]}$, that corresponds to a spin state $\ket{J,M}$ in the continuum limit, can be found easily in terms of a sum over the Clebsch--Gordan coefficients for $\O(3)$, for any suitable values of $\{j'_i\}$:
\begin{equation}
    \label{eq:projectToJM}
    \cO^{J,M}_{[j'_2,\dots,j'_{(N-1)}]}
    =\sum_{\{m_i\}}\sum_{\{m'_i\}}
    \wt{p}_{m_1,\dots,m_N}
    C^{j'_2,m'_2}_{1,m_2;1,m_1}
    \cbr*{\prod_{k=3}^{N-1}
        C^{j'_k,m'_k}_{1,m_k;j'_{(k-1)},m'_{(k-1)}}
    }
    C^{J,M}_{1,m_N;j'_{N-1},m'_{N-1}}\,,
\end{equation}
where the sums over $m_i$ (with $i=1,\dots,N$) are from $-1$ to $+1$, and the sums over $m'_i$ (with $i=2,\dots(n-1)$) are from $-j_i'$ to $+j_i'$. 
Here we denote by $\wt{p}_{m_1,\dots,m_N}$ either $\wt{\alpha}_{m_1,\dots,m_N}$ or $\wt{\beta}_{m_1,\dots,m_N;\{r,s\}}$ at fixed $\{r,s\}$ depending on whether the final state should be neutral or charged under the custodial symmetry. 

On the lattice it also makes sense to distinguish channels with the same continuum spin $J$ which transform under different irreps of the octahedral group. For a fixed set of values of $\{j'_i\}$ in \cref{eq:projectToJM}, we can then further project to a given lattice irrep $\Lambda$, and `row' of said irrep, $\lambda\in\{1,\dots,\dim(\Lambda)\}$, as follows:
\begin{equation}
    \label{eq:projectToIrrep}
    \cO^{J,\Lambda}_{[j'_2,\dots,j'_{(N-1)}];\lambda}
    =\sum_{M=-J}^{J}\mathcal{S}^{J,M}_{\Lambda,\lambda}
    \cO^{J,M}_{[j'_2,\dots,j'_{(N-1)}]}\,,
\end{equation}
where the `subduction coefficients' $\mathcal{S}^{J,M}_{\Lambda,\lambda}$ can be derived in terms of the $\SO(3)$ and $O_h$ Clebsch--Gordan coefficients, and are given explicitly in \cite[IV.A]{dudek2010}. The results up to spin-2 (omitting the $j'_i$ labels for simplicity) are then 
\begin{multline}
    \label{eq:explicitIrreps}
    \cO^{J=0,\Lambda=A_1}=\cO^{J=0,M=0}
    \qquad
    \cO^{J=1,\Lambda=T_1}=\pmat{\cO^{J=1,M=1}\\\cO^{J=1,M=0}\\\cO^{J=1,M=-1}}\,,
    \\
    \cO^{J=2,\Lambda=T_2}=
    \pmat{\cO^{J=2,M=1}\\(\cO^{J=2,M=2}-\cO^{J=2,M=-2})/\sqrt{2}\\\cO^{J=2,M=-1}}
    \qquad
    \cO^{J=2,\Lambda=E}=
    \pmat{\cO^{J=2,M=0}\\(\cO^{J=2,M=2}+\cO^{J=2,M=-2})/\sqrt{2}}.
\end{multline}
The results can easily be extended for $J\geq 3$, and since this projection does not lose information about the total continuum spin $J$, then for a given irrep, the operators obtained via this procedure do not mix with higher-spin states in the continuum limit.

For any fixed number $N$ of lattice derivatives, it is then simple to iterate over all possible combinations of $\{j'_i\}$ in \cref{eq:projectToJM}, and thus create a large basis of operators up to a given maximum spin. \footnote{note about maximum spin/mass here}
Finally, the operators obtained in \cref{eq:explicitIrreps} can be simply projected to their $P=\pm 1$ parity components, and in the custodially-neutral case, also to $C=\pm 1$ charge-parity.

This basic procedure can also be used to obtain pure-gauge operators in the various channels (see \cite{wurtz2015} and \cite{wurtz2013} for explicit examples) by considering as the basis of operators closed loops in the space of gauge fields. Using the fact that any such loop may be rewritten in terms of the trace over a local product of plaquettes, we can follow an identical procedure to the one abve, substituting the $\wt{p}_{m_1,\dots,m_N}$ in \eqref{eq:projectToJM} with
\begin{multline}
    \wt{\theta}_{m_1,\dots,m_N; \{r_1,\dots,r_Q\}}(x) = \tr\Big[(D_{m_{N}}\dots D_{m_{N-r_Q}}U_{m_{N-1},m_N})(x)
    \dots (D_{m_{r_1}}\dots D_{m_{3}}U_{m_{2},m_1})(x)\Big]\,.
\end{multline}
That is, instead of acting on scalars with strings of derivatives, we act on a fixed number $Q$ of plaquettes, then take the trace.
\EDil{need to check this expression, don't think it's quite right}

For the adjoint-scalar case, we consider also a fixed number $Q$ of insertions of the scalar field into the trace.
\EDil{not sure how to write this neatly either....}
% , i.e.
% \begin{equation}
%     \wt{\omega}_{m_1,\dots,m_N; \{r_1,\dots,r_Q\}}(x) = \frac{1}{\sqrt{\tr(\phi^2)^{Q}}} \tr(\phi)
% \end{equation}
% and can be generalised easily to the adjoint-scalar case, replacing the `strings' of links dressed by scalars with traces over closed loops of links with insertions of scalar fields). That is, to generate pure-gauge operators we would replace the $\wt{p}_{m_1,\dots,m_n}$ in \eqref{eq:projectToJM} with 
% \begin{equation}
%     \wt\theta_{m_1,\dots,m_n}=\dots
% \end{equation}

To further increase the operator basis, we also perform APE-smearing on the scalar fields and stout-smearing on the links, and consider scattering states constructed from products of the basic operators defined as linear combinations of $\wt{\alpha}$ and $\wt{\beta}$ operators.


==> extra/draftintro.tex <==
\section{Introduction}

\section{FMS mechanism}

\section{Fundamental spectroscopy}

\section{Conclusions}
